Edge-centric Optimization of Multi-modal ML-driven eHealth Applications

Smart eHealth applications deliver personalized and preventive digital healthcare services to clients through remote sensing, continuous monitoring, and data analytics. Smart eHealth applications sense input data from multiple modalities, transmit the data to edge and/or cloud nodes, and process the data with compute intensive machine learning (ML) algorithms. Run-time variations with continuous stream of noisy input data, unreliable network connection, computational requirements of ML algorithms, and choice of compute placement among sensor-edge-cloud layers affect the efficiency of ML-driven eHealth applications. In this chapter, we present edge-centric techniques for optimized compute placement, exploration of accuracy-performance trade-offs, and cross-layered sense-compute co-optimization for ML-driven eHealth applications. We demonstrate the practical use cases of smart eHealth applications in everyday settings, through a sensor-edge-cloud framework for an objective pain assessment case study.

==> Figures/plot.tex <==
\begin{figure}[t]
\pgfplotsset{every x tick label/.append style={font=\tiny, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\tiny, xshift=0.5ex}}
\usetikzlibrary{patterns}
\pgfplotsset{compat=1.11,
	/pgfplots/ybar legend/.style={
		/pgfplots/legend image code/.code={%
			\draw[##1,/tikz/.cd,yshift=-1mm]
			(5mm,2mm) rectangle (2pt,0.2em);},
	},
}
\centering
\begin{subfigure}[b]{\textwidth}
\centering

\begin{tikzpicture}
\begin{axis}[
ybar=2pt,
enlarge x limits={abs=0.6},
ymin=0,
width  = 9.5cm,
height = 4cm,
bar width=8pt,
grid=major,
ylabel={\normalsize Latency(sec)},
xticklabel style={rotate=0, font=\small},
xtick = data,
ylabel near ticks,
table/header=false,
every node near coord/.append style={font=\tiny},
table/row sep=\\,
xticklabels from table={
	 \\
	 \\
	 \\
	 \\
	 \\
	 \\
}{[index]0},
legend columns=3,
enlarge y limits={value=.4,upper},
legend style={at={(0.5,.99)},anchor=north, font=\small},
]
\addplot [draw=black,pattern=horizontal lines] table[x expr=\coordindex,y index=0]{0.189038\\0.189038\\0.189038\\0.121628\\0.121628\\0.121628\\};
\addplot [draw=black,fill=black]  table[x expr=\coordindex,y index=0,red]{0.410974\\0.039724\\0.037849\\0.20681\\0.021185\\0.0202475\\};
\addplot [draw=black,fill=gray] table[x expr=\coordindex,y index=0]{0.137094\\0.133134\\0.133114\\0.069862\\0.067585\\0.0675735\\}; %NTT 256-512-1024
\legend{Local, Cloud, Partial}
\pgfplotsinvokeforeach{0,1,2,3}{\coordinate(l#1)at(axis cs:#1,0);}
\end{axis}
\draw[thick] (3.95,0) -- (3.95,1.8);
\end{tikzpicture}
\vspace{-3mm}
\caption{Stress Monitoring} \label{fig:Stress}
\end{subfigure}
\begin{subfigure}[b]{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
ybar=2pt,
grid=major,
enlarge x limits={abs=0.6},
ymin=0,
width  = 9.5cm,
height = 4cm,
bar width=8pt,
ylabel={\normalsize Latency(sec)},
xticklabel style={rotate=0, font=\small},
xtick = data,
ylabel near ticks,
table/header=false,
every node near coord/.append style={font=\tiny},
table/row sep=\\,
xticklabels from table={
	 \\
	 \\
	 \\
	 \\
	 \\
	 \\
}{[index]0},
legend columns=3,
enlarge y limits={value=.4,upper},
legend style={at={(0.5,.99)},anchor=north, font=\small}
]
\addplot [draw=black,pattern=horizontal lines] table[x expr=\coordindex,y index=0]{7.25\\7.25\\7.25\\5.7\\5.7\\5.7\\}; %NTT_SA 256-512-1024
\addplot [draw=black,fill=black]  table[x expr=\coordindex,y index=0,red]{13.327\\1.15\\1.0885\\6.895\\0.856\\0.8255\\};
\addplot [draw=black,fill=gray] table[x expr=\coordindex,y index=0]{16.023\\3.846\\3.7845\\8.28\\2.241\\2.2105\\}; %NTT 256-512-1024
%\legend{Local, Cloud, Partial}
\pgfplotsinvokeforeach{0,1,2,3}{\coordinate(l#1)at(axis cs:#1,0);}
\end{axis}
\draw[thick] (3.95,0) -- (3.95,2.9);
%\node[below] at (2.1,-0.5) {(1) High sampling rate};
%\node[below] at (6.0,-0.5) {(2) Low sampling rate};
\end{tikzpicture}
\vspace{-3mm}
\caption{Fall Detection} \label{fig:Fall}
\end{subfigure}

\begin{subfigure}[b]{\textwidth}
\centering
\begin{tikzpicture}
\begin{axis}[
ybar=2pt,
grid=major,
enlarge x limits={abs=0.6},
ymin=0,
width  = 9.5cm,
height = 4cm,
bar width=8pt,
ylabel={\normalsize Latency(sec)},
xticklabel style={rotate=0, font=\small},
xtick = data,
ylabel near ticks,
table/header=false,
every node near coord/.append style={font=\tiny},
table/row sep=\\,
xticklabels from table={
	Low\\
	Med\\
	High\\
	Low\\
	Med\\
	High\\
}{[index]0},
legend columns=3,
enlarge y limits={value=.4,upper},
legend style={at={(0.5,.99)},anchor=north, font=\small},
]
\addplot [draw=black,pattern=horizontal lines] table[x expr=\coordindex,y index=0]{11.394\\11.394\\11.394\\6.564\\6.564\\6.564\\}; %NTT_SA 256-512-1024
\addplot [draw=black,fill=black]  table[x expr=\coordindex,y index=0,red]{25.58\\2.414\\2.297\\24.598\\1.432\\1.315\\};
\addplot [draw=black,fill=gray] table[x expr=\coordindex,y index=0]{10.222\\10.1131\\10.11255\\5.265\\5.1561\\5.15555\\}; %NTT 256-512-10
%\legend{Local, Cloud, Partial}
\pgfplotsinvokeforeach{0,1,2,3}{\coordinate(l#1)at(axis cs:#1,0);}
\end{axis}
\draw[thick] (3.95,0) -- (3.95,2.9);
\node[below] at (2.1,-0.5) {(1) High sampling rate};
\node[below] at (6.0,-0.5) {(2) Low sampling rate};
\end{tikzpicture}
\vspace{-1.5mm}
\caption{Pain Monitoring} \label{fig:Fall}
\end{subfigure}
\caption{Cross-Layer exploration for health monitoring applications.}
\vspace{-5mm}
\label{Exploration}
\end{figure}
